XENON1T Dark Matter Data Analysis: Signal Reconstruction, Calibration and Event Selection

The XENON1T experiment at the Laboratori Nazionali del Gran Sasso is the most sensitive direct detection experiment for dark matter in the form of weakly interacting particles (WIMPs) with masses above $6\,$GeV/$c^2$ scattering off nuclei. The detector employs a dual-phase time projection chamber with 2.0 metric tons of liquid xenon in the target. A one metric $\mathrm{ton}\times\mathrm{year}$ exposure of science data was collected between October 2016 and February 2018. This article reports on the performance of the detector during this period and describes details of the data analysis that led to the most stringent exclusion limits on various WIMP-nucleon interaction models to date. In particular, signal reconstruction, event selection and calibration of the detector response to nuclear and electronic recoils in XENON1T are discussed.

==> Calibrations.tex <==
\section{Calibration data and the determination of signal and background regions in WIMP searches}
\label{sec:Calibration}
%\subsection{Monoenergetic lines in detector}
%\label{subsec:EnergyScale}
%Multiple monoenergetic peaks exist in XENON1T detector. These monoenergetic lines are utilized for detector calibration. $^{83m}$Kr calibrations are done periodically in science run 1. With monoenergetic lines in background, these are used to monitor the light and charge yield stability over time. With an energy range from 9(41)\,keV to 5.5\,MeV, light(charge) yield shows a good stability within 0.18\%(1.4\%) for 1 $\sigma$ deviation, as shown in Fig.  \ref{fig:ly_cy_stability}. The small increase in charge yield is not understood yet and still under investigation. We tested if a potential correction of charge yield increase would affect our analysis and it shows negligible difference, we therefore didn't apply this correction in our analysis.

%\begin{figure}[h]
%  \centering
  %\subfloat[Light yield stability in Science Run1.]
%  {\includegraphics[width=0.48\textwidth]{Calibrations/combined_ly_sr1_mean_offset_171222.png}}\label{fig:ly_stability}
%  \hfill
  %\subfloat[Charge yield stability in Science Run 1.]
%  {\includegraphics[width=0.48\textwidth]{Calibrations/combined_cy_sr1_mean_offset_171222.png}}\label{fig:cy_stability}
%  \caption{Relative signal detection stability throughout science run 1. Upper panel is light yield stability and lower panel is charge yield stability, monitored by monoenergetic lines ranging from 9(41)\,keV to 5.5\,MeV.}
%  \label{fig:ly_cy_stability}
%\end{figure}

% should we use the one from SR1 in PAX 680, https://xe1t-wiki.lngs.infn.it/lib/exe/detail.php?id=xenon%3Axenon1t%3Aanalysis%3Aplots&media=xenon:xenon1t:wittweg:energy_resolution_he_pax_v680_hax_v240_feb17tofeb18.png, or the updated one in PAX 6.10.0, with a better resolution? https://xe1t-wiki.lngs.infn.it/lib/exe/fetch.php?cache=&media=xenon:xenon1t:chiara:double_beta:energy_cal:resolution_update.png
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.45\textwidth]{Calibrations/energy_resolution_comp_pax680.png}
%    \caption{Energy resolution from different detectors. Black dot is XENON1T detector under 81 V/cm(this work).The other points are from \cite{pandax_2_ucla, xe100_instru, lux_analy_paper_2017, exo_II_search_2018}. 
    %Cyan dot is EXO Phase II\cite{exo_II_search_2018}, fitted by an empirical function. Green dot is PandaX\cite{pandax_2_ucla}, yellow dot is XENON100 detector\cite{xe100_instru}, blue dot is LUX detector\cite{lux_analy_paper_2017}.
%    }
%    \label{fig:energyresolution}
%\end{figure}

%\subsection{Calibrations for Discrimination}
%\label{subsec:discrimination_calibration}
%ER leakage note? https://xe1t-wiki.lngs.infn.it/doku.php?id=xenon:xenon1t:analysis:sciencerun1:anomalous_background_update
%\begin{itemize}
%    \item Leakage Fraction plot
%    \item Compare to Plot of leakage fraction from XENON100
%\end{itemize}

Two external neutron sources are deployed for NR calibration in XENON1T. $^{241}$AmBe source and DD neutron generator~\cite{ng_rafael_2017}, which are ($\alpha$, n) reaction and deuteron deuteron fusion, are performed with 30 days and 1.9 days exposure separately and are both contributing to NR response calibration as shown in Fig. \ref{fig:nr_cali_sr1}. A set of quality cuts are applied to select pure NR events which forms NR band. NR median as well as NR $\pm$2 $\sigma$ quantile lines are extracted from NR band, where region between -2 $\sigma$ quantile and median are defined as NR signal reference region.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1\linewidth]{Calibrations/band_plots_blind_sr1_nr.pdf}
    \caption{NR band calibrated by both neutron generator and $^{241}$AmBe source. The black dots are neutron events from these two sources in SR1. Red solid line is median line of NR band, red dashed lines are $\pm$2 $\sigma$ quantile lines of NR band. Blue solid line is median line of ER band, see figure \ref{fig:er_cali_sr1}.}
    \label{fig:nr_cali_sr1}
\end{figure}

A dissolved $^{220}$Rn source is used to calibrate ER events. As detector size is increasing, internal calibration sources are preferred for ER calibration due to the short range of $\beta$ electron or gamma rays. The primary utility of $^{220}$Rn decay chain is the beta decay of $^{212}$Pb, which has Q value of 569.9 keV with a branching ratio of 11.9\%~\cite{bnl_nndc}. The half-life of $^{212}$Pb beta decay is 10.64 h, the longest in the whole decay chain, is long enough to distribute uniformly in the detector and short enough that all introduced activity can vanish within one week. Seven $^{220}$Rn calibrations from different periods in SR0 and SR1 show good stability of ER response. ER band, defined from $^{220}$Rn calibration, is shown in figure \ref{fig:er_cali_sr1}. Slices in S1 in both ER and NR band can be described as Gaussian\cite{xe1t_long_analysis_2}. The leakage fraction of ER events into NR signal reference region is 0.3\%.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1\linewidth]{Calibrations/band_plots_blind_sr1_er.pdf}
    \caption{ER band calibrated by $^{220}$Rn source in SR1. Black dots are $^{220}$Rn events. Blue solid line is median line of ER band, blue dashed lines are $\pm$2 $\sigma$ quantile lines of ER band. The red line is median line from NR band, see figure \ref{fig:nr_cali_sr1}.}
    \label{fig:er_cali_sr1}
\end{figure}



